Non-statistical rational maps

We show that in the family of degree $d\geq 2$ rational maps of the Riemann sphere, the closure of strictly postcritically finite maps contains a (relatively) Baire generic subset of maps displaying maximal non-statistical behavior: for a map $f$ in this generic subset, the set of accumulation points of the sequence of empirical measures of almost every point in the phase space is the largest possible one that is, the set of all $f$-invariant measures. The proofs is based on a transversality argument which allows us to control the behavior of the orbits of critical points for maps close to strictly postcritically finite rational maps and also a new concept developed in the author's PhD thesis, that we call statistical bifurcation.

==> references.tex <==
@article{przytycki1996porosity,
  title={Porosity of Collet-Eckmann Julia sets},
  author={Przytycki, Feliks and Rohde, Steffen},
  journal={arXiv preprint math/9604234},
  year={1996}
}

@InCollection{milnor2006lattes,
 Author = {John {Milnor}},
 Title = {{On Latt\`es maps.}},
 BookTitle = {{Dynamics on the Riemann sphere. A Bodil Branner Festschrift}},
 ISBN = {3-03719-011-6/hbk},
 Pages = {9--43},
 Year = {2006},
 Publisher = {Z\"urich: European Mathematical Society Publishing House},
 Language = {English},
 MSC2010 = {37F10 37-02 37-03 30D05},
 Zbl = {1235.37015}
}

@inproceedings{przytycki2007statistical,
  title={Statistical properties of topological Collet-Eckmann maps},
  author={Przytycki, Feliks and Rivera-Letelier, Juan},
  booktitle={Annales scientifiques de l'Ecole normale sup{\'e}rieure},
  volume={40},
  number={1},
  pages={135--178},
  year={2007}
}

@article{talebi20,
 author = {Amin Talebi},

 title = {Statistical stability and non-statistical dynamics, manuscript},

 year = {2020}
}



@article{Singer,
 author = {David Singer},
 journal = {SIAM Journal on Applied Mathematics},
 number = {2},
 pages = {260--267},
 publisher = {Society for Industrial and Applied Mathematics},
 title = {Stable Orbits and Bifurcation of Maps of the Interval},
 volume = {35},
 year = {1978}
}

@article{Guck79,
author = {Guckenheimer, John},
year = {1979},
month = {06},
pages = {133-160},
title = {Sensitive dependence to initial conditions for one dimensional maps},
volume = {70},
journal = {Commun.Math.Phys.},
doi = {10.1007/BF01982351}
}

@article{crovisier2020empirical,
  title={Empirical measures of partially hyperbolic attractors},
  author={Crovisier, Sylvain and Yang, Dawei and Zhang, Jinhua},
  journal={Communications in Mathematical Physics},
  pages={1--40},
  year={2020},
  publisher={Springer}
}
@article{Berger-Biebler2020,
  title={Emergence of wandering stable components},
  author={Berger, Pierre and Biebler, Sebastien},
  journal={arXiv:2001.08649},
    year={2020},

}

@article{KNS2019,
  title={Emergence via non-existence of averages},
  author={Kiriki, Shin and Nakano, Yushi and Soma, Teruhiko },
  journal={arXiv:1904.03424},
   year={2019},
}

@Article{bonk1996bounds,
 Author = {Mario {Bonk} and William {Cherry}},
 Title = {{Bounds on spherical derivatives for maps into regions with symmetries.}},
 FJournal = {{Journal d'Analyse Math\'ematique}},
 Journal = {{J. Anal. Math.}},
 ISSN = {0021-7670; 1565-8538/e},
 Volume = {69},
 Pages = {249--274},
 Year = {1996},
 Publisher = {Springer, Berlin/Heidelberg; Hebrew University Magnes Press, Jerusalem},
 Language = {English},
 MSC2010 = {30D45 30F45},
 Zbl = {0881.30029}
}
@inproceedings{przytycki2001porosity,
  title={Porosity of Julia sets of non-recurrent and parabolic Collect-Eckmann rational functions},
  author={Przytycki, F. and Urbanski, M.},
  booktitle={Annales-Academiae Scientiarum Fennicae series A1 mathematica},
  volume={26},
  number={1},
  pages={125--154},
  year={2001},
  organization={Academia Scientiarum Fenica}
}

@Article{Takens1994,
author="Takens, Floris",
title="Heteroclinic attractors: Time averages and moduli of topological conjugacy",
journal="Boletim da Sociedade Brasileira de Matem{\'a}tica - Bulletin/Brazilian Mathematical Society",
year="1994",
month="Mar",
day="01",
volume="25",
number="1",
pages="107--120",
abstract="In this paper we consider attracting heteroclinic cycles. We recall that these cycles usually have no S.B.R. measure. This is related with the fact that certain time averages do not converge. We obtain a topological interpretation of the asymptotic properties of these non-converging time averages. In terms of these asymptotic properties we obtain a complete set of moduli for the attracting heteroclinic cycles.",
issn="1678-7714",
doi="10.1007/BF01232938",
url="https://doi.org/10.1007/BF01232938"
}


@Article{Baladi2015,
author="Baladi, Viviane
and Benedicks, Michael
and Schnellmann, Daniel",
title="Whitney--H{\"o}lder continuity of the SRB measure for transversal families of smooth unimodal maps",
journal="Inventiones mathematicae",
year="2015",
month="Sep",
day="01",
volume="201",
number="3",
pages="773--844",
}
@article{AB09,
author = {Avila, Artur and Bochi, Jairo},
year = {2009},
month = {12},
pages = {},
title = {Nonuniform Hyperbolicity, Global Dominated Splittings and Generic Properties of Volume-Preserving Diffeomorphisms},
volume = {364},
journal = {Transactions of the American Mathematical Society},
doi = {10.1090/S0002-9947-2012-05423-7}
}

@article  {Y95,
    AUTHOR = {J.-C., Yoccoz},
     TITLE = {A proof of {J}akobson's Theorem},
		JOURNAL = {This volume},
}

@article  {berhen,
    AUTHOR = {Berger, P.},
     TITLE = {Abundance of non-unformly hyperbolicH�non-like endomorphisms},
		JOURNAL = {Paper under review},
}

@book {PT93,
    AUTHOR = {Palis, J. and Takens, F.},
     TITLE = {Hyperbolicity and sensitive chaotic dynamics at homoclinic
              bifurcations},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {35},
      NOTE = {Fractal dimensions and infinitely many attractors},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1993},
}

@article {GS97,
    AUTHOR = {Graczyk, J. and {\'S}wiatek, G.},
     TITLE = {Generic hyperbolicity in the logistic family},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {146},
      YEAR = {1997},
    NUMBER = {1},
     PAGES = {1--52},
}
@article {Lorenz,
    AUTHOR = {Lorenz, E. N.},
     TITLE = {Deterministic Nonperiodic Flow},
   JOURNAL = {J. Atmos. Sci.},
    VOLUME = {20},
      YEAR = {1963},
      PAGES = {130--141},
}


@article {Ur95,		
    AUTHOR = {Ures, R.},
     TITLE = {On the approximation of {H}\'enon-like attractors by
              homoclinic tangencies},
   JOURNAL = {Ergodic Theory Dynam. Systems},
    VOLUME = {15},
      YEAR = {1995},
    NUMBER = {6},
     PAGES = {1223--1229},
   }


@preamble{
   "\def\polhk#1{\setbox0=\hbox{#1}{\ooalign{\hidewidth
    \lower1.5ex\hbox{`}\hidewidth\crcr\unhbox0}}} "
}
@article {Ly97,
    AUTHOR = {Lyubich, M.},
     TITLE = {Dynamics of quadratic polynomials. {I}, {II}},
   JOURNAL = {Acta Math.},
    VOLUME = {178},
      YEAR = {1997},
    NUMBER = {2},
     PAGES = {185--247, 247--297},
}

@article{BL91,
     author = {Blokh, A. M. and Lyubich, Mikhail Yu.},
     title = {Measurable dynamics of $S$-unimodal maps of the interval},
     journal = {Annales scientifiques de l'\'Ecole Normale Sup\'erieure},
     publisher = {Elsevier},
     volume = {Ser. 4, 24},
     number = {5},
     year = {1991},
     pages = {545-573},
     doi = {10.24033/asens.1636},
     zbl = {0790.58024},
     mrnumber = {93f:58132},
     language = {en},
     
}
@article {Ta11,
    AUTHOR = {Takahasi, H.},
     TITLE = {Abundance of non-uniform hyperbolicity in bifurcations of
              surface endomorphisms},
   JOURNAL = {Tokyo J. Math.},
    VOLUME = {34},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {53--113},
}
@article {YW08,
    AUTHOR = {Wang, Q. and Young, L.-S.},
     TITLE = {Toward a theory of rank one attractors},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {167},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {349--480},
}
@article {MV93,
    AUTHOR = {Mora, L. and Viana, M.},
     TITLE = {Abundance of strange attractors},
   JOURNAL = {Acta Math.},
    VOLUME = {171},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {1--71},
}

@article {WY01,
    AUTHOR = {Wang, Q. and Young, L.-S.},
     TITLE = {Strange attractors with one direction of instability},
   JOURNAL = {Comm. Math. Phys.},
    VOLUME = {218},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {1--97},
 }


@article {Ja81,
    AUTHOR = {Jakobson, M. V.},
     TITLE = {Absolutely continuous invariant measures for one-parameter
              families of one-dimensional maps},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {81},
      YEAR = {1981},
    NUMBER = {1},
     PAGES = {39--88},
}
@article {Re86,
    AUTHOR = {M. Rees},
     TITLE = {Positive measure sets of ergodic rational maps},
   JOURNAL = {Ann. Sci. \'Ecole Norm. Sup. (4)},
  FJOURNAL = {Annales Scientifiques de l'\'Ecole Normale Sup\'erieure.
              Quatri\`eme S\'erie},
    VOLUME = {19},
      YEAR = {1986},
    NUMBER = {3},
     PAGES = {383--407},
}
@article {PY09,
    AUTHOR = {J. Palis and J.-C. Yoccoz},
     TITLE = {Non-uniformly hyperbolic horseshoes arising from bifurcations
              of {P}oincar\'e heteroclinic cycles},
   JOURNAL = {Publ. Math. Inst. Hautes \'Etudes Sci.},
    NUMBER = {110},
      YEAR = {2009},
     PAGES = {1--217},
 
}


@article {B11,
    AUTHOR = {Berger, P.},
     TITLE = {Abundance of non-uniformly hyperbolic {H}\'enon like endomorphisms},
		JOURNAL = {This voume},
}

@incollection {Yoc-Her,
    AUTHOR = {Herman, Michael},
     TITLE = {An example of non-convergence of Birkhoff sums},
 BOOKTITLE = {Notes inachev\'ees de Michael R. Herman s\'electionn\'ees par Jean-Christophe Yoccoz},
     PAGES = {183--185},
 PUBLISHER = {Soci\'et\'e Math\'ematique de France},
      YEAR = { 2018},
   
}


@incollection {Hu91,
    AUTHOR = {Hubbard, J. H.},
     TITLE = {Local connectivity of {J}ulia sets and bifurcation loci: three
              theorems of {J}.-{C}. {Y}occoz},
 BOOKTITLE = {Topological methods in modern mathematics ({S}tony {B}rook,
              {NY}, 1991)},
     PAGES = {467--511},
 PUBLISHER = {Publish or Perish, Houston, TX},
      YEAR = {1993},
   MRCLASS = {58F23 (28A80 30C10 58F12)},
  MRNUMBER = {1215974 (94c:58172)},
MRREVIEWER = {Christoph Bandt},
}

@article {ALMdM,
    AUTHOR = {Avila, A. and Lyubich, M. and de Melo, W.},
     TITLE = {Regular or stochastic dynamics in real analytic families of
              unimodal maps},
   JOURNAL = {Invent. Math.},
    VOLUME = {154},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {451--550},
}
@article {AM03,
    AUTHOR = {Avila, A. and Moreira, C. G.},
     TITLE = {Statistical properties of unimodal maps: smooth families with
              negative {S}chwarzian derivative},
      NOTE = {Geometric methods in dynamics. I},
   JOURNAL = {Ast\'erisque},
    NUMBER = {286},
      YEAR = {2003},
     PAGES = {xviii, 81--118},
}
@article {L02,
    AUTHOR = {Lyubich, M.},
     TITLE = {Almost every real quadratic map is either regular or
              stochastic},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {156},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {1--78},
}

@article {AKLS,
    AUTHOR = {Avila, A.r and Kahn, J. and Lyubich, M. and Shen,
              W.},
     TITLE = {Combinatorial rigidity for unicritical polynomials},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {170},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {783--797},
  }
@book {Mi06,
    AUTHOR = {Milnor, J.},
     TITLE = {Dynamics in one complex variable},
    SERIES = {Annals of Mathematics Studies},
    VOLUME = {160},
   EDITION = {Third},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {2006},
}
@incollection {Mi92,
    AUTHOR = {Milnor, J.},
     TITLE = {Local connectivity of {J}ulia sets: expository lectures},
 BOOKTITLE = {The {M}andelbrot set, theme and variations},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {274},
     PAGES = {67--116},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2000},
   MRCLASS = {37F50 (30D05 37-02)},
  MRNUMBER = {1765085 (2001b:37073)},
}

@article {Henon,
    AUTHOR = {H{\'e}non, M.},
     TITLE = {A two-dimensional mapping with a strange attractor},
   JOURNAL = {Comm. Math. Phys.},
    VOLUME = {50},
      YEAR = {1976},
    NUMBER = {1},
     PAGES = {69--77},
}

@incollection {BP06,
    AUTHOR = {Barreira, L. and Pesin, Y.},
     TITLE = {Smooth ergodic theory and nonuniformly hyperbolic dynamics},
 BOOKTITLE = {Handbook of dynamical systems. {V}ol. 1{B}},
     PAGES = {57--263},
      NOTE = {With an appendix by Omri Sarig},
 PUBLISHER = {Elsevier B. V., Amsterdam},
      YEAR = {2006},
}

@book {Sh71,
    AUTHOR = {Shub, M.},
     TITLE = {Topologically transitive diffeomorphisms of T4},
    SERIES = {Lecture Notes in Mathematics, Vol. 206},
    EDITOR = {Chillingworth, David},
 PUBLISHER = {Springer-Verlag, Berlin-New York},
      YEAR = {1971},
     PAGES = {39�-40},
}
@article {LY,
    AUTHOR = {Ledrappier, F. and Young, L.-S.},
     TITLE = {The metric entropy of diffeomorphisms. {I}. {C}haracterization
              of measures satisfying {P}esin's entropy formula},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {122},
      YEAR = {1985},
    NUMBER = {3},
     PAGES = {509--539},
  }

@article{ledrappier_1981, title={Some properties of absolutely continuous invariant measures on an interval}, volume={1}, DOI={10.1017/S0143385700001176}, number={1}, journal={Ergodic Theory and Dynamical Systems}, publisher={Cambridge University Press}, author={Ledrappier, François}, year={1981}, pages={77–93}}

@article {Ts93,
    AUTHOR = {Tsujii, M.},
     TITLE = {A proof of {B}enedicks-{C}arleson-{J}acobson theorem},
   JOURNAL = {Tokyo J. Math.},
    VOLUME = {16},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {295--310},
   }


@incollection {Lu00,
    AUTHOR = {Luzzatto, S.},
     TITLE = {Bounded recurrence of critical points and {J}akobson's
              theorem},
 BOOKTITLE = {The {M}andelbrot set, theme and variations},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {274},
     PAGES = {173--210},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2000},
 }



@article {Ts932,
    AUTHOR = {Tsujii, M.},
     TITLE = {Positive {L}yapunov exponents in families of one-dimensional
              dynamical systems},
   JOURNAL = {Invent. Math.},
    VOLUME = {111},
      YEAR = {1993},
    NUMBER = {1},
     PAGES = {113--137},
}




@article {BC91,
    AUTHOR = {Benedicks, M. and Carleson, L.},
     TITLE = {The dynamics of the {H}\'enon map},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {133},
      YEAR = {1991},
    NUMBER = {1},
     PAGES = {73--169},
}
			
			
			
			
			
			
			
@article {Yurch,
    AUTHOR = {Pesin, Ya. B. and Yurchenko, A. A.},
     TITLE = {Some physical models described by the reaction-diffusion
              equation, and coupled map lattices},
   JOURNAL = {Uspekhi Mat. Nauk},
    VOLUME = {59},
      YEAR = {2004},
    NUMBER = {3(357)},
     PAGES = {81--114},

}
@book {QXZ,
    AUTHOR = {Qian, M. and Xie, J.-S. and Zhu, S.},
     TITLE = {Smooth ergodic theory for endomorphisms},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1978},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2009},
     PAGES = {xiv+277},
}
@article {BY, AUTHOR = {Benedicks, M. and Young, L.-S.}, TITLE = {Sina\u\i-{B}owen-{R}uelle measures for certain {H}\'enon maps}, JOURNAL = {Invent. Math.}, VOLUME = {112}, YEAR = {1993}, NUMBER = {3}, PAGES = {541--576},
}
@article {MY10,
    AUTHOR = {Moreira, C. G. and Yoccoz, J.-C.},
     TITLE = {Tangences homoclines stables pour des ensembles hyperboliques
              de grande dimension fractale},
   JOURNAL = {Ann. Sci. \'Ec. Norm. Sup\'er. (4)},
    VOLUME = {43},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {1--68},
 
}

@article {GuguYo,
    AUTHOR = {de A. Moreira, C. G. T. and Yoccoz, J.-C.},
     TITLE = {Stable intersections of regular {C}antor sets with large
              {H}ausdorff dimensions},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {154},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {45--96},
}

@article {Roh,
    AUTHOR = {Rohlin, V. A.},
     TITLE = {On the fundamental ideas of measure theory},
   JOURNAL = {Amer. Math. Soc. Translation},
    VOLUME = {1952},
      YEAR = {1952},
    NUMBER = {71},
     PAGES = {55},
 }
@article {CE80,
    AUTHOR = {Collet, P. and Eckmann, J.-P.},
     TITLE = {On the abundance of aperiodic behaviour for maps on the
              interval},
   JOURNAL = {Comm. Math. Phys.},
    VOLUME = {73},
      YEAR = {1980},
    NUMBER = {2},
     PAGES = {115--160},
 }

@article {CE83,
    AUTHOR = {Collet, P. and Eckmann, J.-P.},
     TITLE = {Positive {L}iapunov exponents and absolute continuity for maps
              of the interval},
   JOURNAL = {Ergodic Theory Dynam. Systems},
    VOLUME = {3},
      YEAR = {1983},
    NUMBER = {1},
     PAGES = {13--46},
 }

@article {BC1,
    AUTHOR = {M. Benedicks and L. Carleson},
     TITLE = {On iterations of $1-ax^2$},
   JOURNAL = {Ann. Math.},
    VOLUME = {122},
      YEAR = {1985},
     PAGES = {1--25},
}
@article {BC2,
    AUTHOR = {M. Benedicks and L. Carleson},
     TITLE = {The dynamics of the {H}\'enon map},
   JOURNAL = {Ann. Math.},
    VOLUME = {133},
      YEAR = {1991},
     PAGES = {73--169},
}
@article {Ro74,
    AUTHOR = {Robinson, C.},
     TITLE = {Structural stability of vector fields},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {99},
      YEAR = {1974},
     PAGES = {154--175},
 }
@ARTICLE{BK13,
   author = {{Berger}, P. and {Kocsard}, A.},
    title = "{Structural stability of the inverse limit of endomorphisms}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1306.6799},
 primaryClass = "math.DS",
     year = 2013,
}


@article {Ro83,
    AUTHOR = {Robinson, C.},
     TITLE = {Bifurcation to infinitely many sinks},
   JOURNAL = {Comm. Math. Phys.},
    VOLUME = {90},
      YEAR = {1983},
    NUMBER = {3},
     PAGES = {433--459},
  }

@article {Mora-viana,
    AUTHOR = {L. Mora and M. Viana},
     TITLE = {Abundance of strange attractors},
   JOURNAL = {Acta. Math.},
    VOLUME = {171},
      YEAR = {1993},
     PAGES = {1--71},
}
@article {BV01,
    AUTHOR = {M. Benedicks and M. Viana},
     TITLE = {Solution of the basin problem for {H}\'enon-like attractors},
   JOURNAL = {Invent. Math.},
    VOLUME = {143},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {375--434},
}

@article {BV,
    AUTHOR = {M. Benedicks and M. Viana},
     TITLE = {Random perturbations and statistical properties of {H}\'enon-like maps},
   JOURNAL = { Annales Inst. Henri Poincar�},
    VOLUME = {23},
      YEAR = {2006},
     PAGES = {713--752},
}

@article {Newhouse,
    AUTHOR = {Newhouse, S. E.},
     TITLE = {Diffeomorphisms with infinitely many sinks},
   JOURNAL = {Topology},
    VOLUME = {12},
      YEAR = {1974},
     PAGES = {9-18},
}

@article {Se03,
    AUTHOR = {Senti, S.},
     TITLE = {Dimension of weakly expanding points for quadratic maps},
   JOURNAL = {Bull. Soc. Math. France},
    VOLUME = {131},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {399--420},
  }
	@article {SeTa13,
    AUTHOR = {Senti, Samuel and Takahasi, Hiroki},
     TITLE = {Equilibrium measures for the {H}\'enon map at the first
              bifurcation},
   JOURNAL = {Nonlinearity},
    VOLUME = {26},
      YEAR = {2013},
    NUMBER = {6},
     PAGES = {1719--1741},
 }
@article {Du94,
    AUTHOR = {Duarte, P.},
     TITLE = {Plenty of elliptic islands for the standard family of area
              preserving maps},
   JOURNAL = {Ann. Inst. H. Poincar\'e Anal. Non Lin\'eaire},
    VOLUME = {11},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {359--409},
  }

@book {Si94,
    AUTHOR = {Sina{\u\i}, Ya. G.},
     TITLE = {Topics in ergodic theory},
    SERIES = {Princeton Mathematical Series},
    VOLUME = {44},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {1994},
     PAGES = {viii+218},
  }

@article {Sa13,
    AUTHOR = {Sarig, Omri M.},
     TITLE = {Symbolic dynamics for surface diffeomorphisms with positive
              entropy},
   JOURNAL = {J. Amer. Math. Soc.},
    VOLUME = {26},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {341--426},
  }

@article {BeCa13,
    AUTHOR = {P. Berger and P. D. Carrasco},
     TITLE = {Non uniformly hyperbolic diffeomorphisms derived from the standard map},
   JOURNAL = {Communication mathematical physics},
      YEAR = {2014},
}
@inproceedings {Ca91,
    AUTHOR = {Carleson, L.},
     TITLE = {The dynamics of non-uniformly hyperbolic systems in two
              variables},
 BOOKTITLE = {Proceedings of the {I}nternational {C}ongress of
              {M}athematicians, {V}ol.\ {I}, {II} ({K}yoto, 1990)},
     PAGES = {1241--1247},
 PUBLISHER = {Math. Soc. Japan, Tokyo},
      YEAR = {1991},
  }

		
@article {RHO80,
    AUTHOR = {Russell, David A. and Hanson, James D. and Ott, Edward},
     TITLE = {Dimension of strange attractors},
   JOURNAL = {Phys. Rev. Lett.},
    VOLUME = {45},
      YEAR = {1980},
    NUMBER = {14},
     PAGES = {1175--1178},
  }
			
@article {Berentropy,
    AUTHOR = {Berger, P.},
     TITLE = {Properties of the maximal entropy measure and geometry of H�non attractors},
   JOURNAL = {arXiv:math.DS},
      YEAR = {2012},
}

@article {bergugu,
    AUTHOR = {P. Berger and C. G. Moreira},
     TITLE = {Nested Cantor sets},
   JOURNAL = {arXiv:math.DS},
      YEAR = {2013},
}


@article {berlam,
    AUTHOR = {Berger, P.},
     TITLE = {Persistence of Laminations},
   JOURNAL = {arXiv:math.DS},
      YEAR = {2008},
}
@article {Y98,
    AUTHOR = {Young, L.-S.},
     TITLE = {Statistical properties of dynamical systems with some
              hyperbolicity},
   JOURNAL = {Ann. of Math. (2)},
    VOLUME = {147},
      YEAR = {1998},
    NUMBER = {3},
     PAGES = {585--650},
  }
@article {Sm,
    AUTHOR = {Smale, S.},
     TITLE = {Differentiable dynamical systems},
   JOURNAL = {Bull. Amer. Math. Soc.},
    VOLUME = {73},
      YEAR = {1967},
     PAGES = {747--817},
  }

@article {YW,
    AUTHOR = {L. S. Young and Q. D. Wang},
     TITLE = {attractors with one direction of instability},
   JOURNAL = {Commun. Math. Phys.},
    VOLUME = {218},
      YEAR = {2001},
     PAGES = {1--97},
}

@article{fort1951points,
  title={Points of continuity of semicontinuous functions},
  author={Fort, Marion K},
  journal={Publ. Math. Debrecen},
  volume={2},
  pages={100--102},
  year={1951}
}

@article{hofbauer1990,
author = "Hofbauer, Franz and Keller, Gerhard",
fjournal = "Communications in Mathematical Physics",
journal = "Comm. Math. Phys.",
number = "2",
pages = "319--337",
publisher = "Springer",
title = "Quadratic maps without asymptotic measure",
url = "https://projecteuclid.org:443/euclid.cmp/1104180141",
volume = "127",
year = "1990"
}

@book {MR1239171,
    AUTHOR = {de Melo, Welington and van Strien, Sebastian},
     TITLE = {One-dimensional dynamics},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results
              in Mathematics and Related Areas (3)]},
    VOLUME = {25},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1993},
     PAGES = {xiv+605},
      ISBN = {3-540-56412-8},
   MRCLASS = {58F03 (58-02 58Fxx)},
  MRNUMBER = {1239171},
MRREVIEWER = {Feliks Przytycki},
       DOI = {10.1007/978-3-642-78043-1},
       URL = {https://doi-org.ezp2.semantak.com/10.1007/978-3-642-78043-1},
}

@Article{CV01,
 Author = {Eduardo {Colli} and Edson {Vargas}},
 Title = {{Non-trivial wandering domains and homoclinic bifurcations.}},
 FJournal = {{Ergodic Theory and Dynamical Systems}},
 Journal = {{Ergodic Theory Dyn. Syst.}},
 ISSN = {0143-3857; 1469-4417/e},
 Volume = {21},
 Number = {6},
 Pages = {1657--1681},
 Year = {2001},
 Publisher = {Cambridge University Press, Cambridge},
 Language = {English},
 MSC2010 = {37G25 37A99 37D05 37E30},
 Zbl = {1080.37059}
}

@Article{KS15,
 Author = {Shin {Kiriki} and Teruhiko {Soma}},
 Title = {{Takens' last problem and existence of non-trivial wandering domains.}},
 FJournal = {{Advances in Mathematics}},
 Journal = {{Adv. Math.}},
 ISSN = {0001-8708},
 Volume = {306},
 Pages = {524--588},
 Year = {2017},
 Publisher = {Elsevier (Academic Press), San Diego, CA},
 Language = {English},
 MSC2010 = {37C29 37C05 37G25 37D20 37D25 37D05},
 Zbl = {1381.37031}
}


@InCollection{HK2,
 Author = {Franz {Hofbauer} and Gerhard {Keller}},
 Title = {{Quadratic maps with maximal oscillation.}},
 BookTitle = {{Algorithms, fractals, and dynamics. Proceedings of the Hayashibara Forum '92: International symposium on new bases for engineering science, algorithms, dynamics, and fractals, Okayama, Japan, November 23-28, 1992 and a symposium on algorithms, fractals, and dynamics, November 30--December 2, 1992, Kyoto, Japan}},
 ISBN = {0-306-45127-1/hbk},
 Pages = {89--94},
 Year = {1995},
 Publisher = {New York, NY: Plenum Press},
 Language = {English},
 MSC2010 = {37E99 28D05 26A18},
 Zbl = {0873.58028}
}

@article{gaunersdorfer1992time,
  title={Time averages for heteroclinic attractors},
  author={Gaunersdorfer, Andrea},
  journal={SIAM Journal on Applied Mathematics},
  volume={52},
  number={5},
  pages={1476--1489},
  year={1992},
  publisher={SIAM}
}

@article{takens1994heteroclinic,
  title={Heteroclinic attractors: time averages and moduli of topological conjugacy},
  author={Takens, Floris},
  journal={Boletim da Sociedade Brasileira de Matem{\'a}tica-Bulletin/Brazilian Mathematical Society},
  volume={25},
  number={1},
  pages={107--120},
  year={1994},
  publisher={Springer}
}

@Article{Kriki&Soma,
 Author = {Shin {Kiriki} and Teruhiko {Soma}},
 Title = {{Takens' last problem and existence of non-trivial wandering domains.}},
 FJournal = {{Advances in Mathematics}},
 Journal = {{Adv. Math.}},
 ISSN = {0001-8708},
 Volume = {306},
 Pages = {524--588},
 Year = {2017},
 Publisher = {Elsevier (Academic Press), San Diego, CA},
 Language = {English},
 MSC2010 = {37C29 37C05 37G25 37D20 37D25 37D05},
 Zbl = {1381.37031}
}

@Article{buff2013perturbations,
 Author = {Xavier {Buff} and Thomas {Gauthier}},
 Title = {{Perturbations des exemples de Latt\`es flexibles.}},
 FJournal = {{Bulletin de la Soci\'et\'e Math\'ematique de France}},
 Journal = {{Bull. Soc. Math. Fr.}},
 ISSN = {0037-9484; 2102-622X/e},
 Volume = {141},
 Number = {4},
 Pages = {603--614},
 Year = {2013},
 Publisher = {Soci\'et\'e Math\'ematique de France (SMF), Paris},
 Language = {English},
 MSC2010 = {37F45 37D05},
 Zbl = {1326.37035}
}
@InCollection{BE09,
 Author = {Xavier {Buff} and Adam {Epstein}},
 Title = {{Bifurcation measure and postcritically finite rational maps.}},
 BookTitle = {{Complex dynamics. Families and friends}},
 ISBN = {978-1-56881-450-6/hbk},
 Pages = {491--512},
 Year = {2009},
 Publisher = {Wellesley, MA: A K Peters},
 Language = {English},
 MSC2010 = {37F10 37F45},
 Zbl = {1180.37056}
}

@article{AV02,
author = {Alves, José and Viana, Marcelo},
year = {2002},
month = {12},
pages = {1-32},
title = {Statistical Stability for Robust Classes of Maps With Non-Uniform Expansion},
volume = {22},
journal = {Ergodic Theory and Dynamical Systems},
doi = {10.1017/S0143385702000019}
}

@article{APV16,
author = {Alves, José and Pumariño, Antonio and Vigil, Enrique},
year = {2016},
month = {12},
pages = {},
title = {Statistical stability for multidimensional piecewise expanding maps},
journal = {Preprint},
doi = {10.1090/proc/13518}
}

@article{ACF10,
     author = {Alves, Jos\'e F. and Carvalho, Maria and Freitas, Jorge Milhazes},
     title = {Statistical stability for H\'enon maps of the Benedicks--Carleson type},
     journal = {Annales de l'I.H.P. Analyse non lin\'eaire},
     publisher = {Elsevier},
     volume = {27},
     number = {2},
     year = {2010},
     pages = {595-637},
     doi = {10.1016/j.anihpc.2009.09.009},
     zbl = {1205.37040},
     mrnumber = {2595193},
     language = {en},
     url = {http://www.numdam.org/item/AIHPC_2010__27_2_595_0}
}

@inbook{AS13,
author = {Alves, José and Soufi, Mohammad},
year = {2013},
month = {04},
pages = {7-24},
title = {Statistical Stability in Chaotic Dynamics},
volume = {54},
isbn = {ISBN 978-3-642-38829-3},
journal = {Springer Proceedings in Mathematics and Statistics},
doi = {10.1007/978-3-642-38830-9_2}
}


@article{T01,
author = {Thunberg, Hans},
year = {2001},
month = {03},
pages = {},
title = {Unfolding of chaotic unimodal maps and the parameter dependence of natural measures},
volume = {14},
journal = {Nonlinearity},
doi = {10.1088/0951-7715/14/2/308}
}

@Article{AMGT17,
 Author = {Matthieu {Astorg} and Thomas {Gauthier} and Nicolae {Mihalache} and Gabriel {Vigny}},
 Title = {{Collet, Eckmann and the bifurcation measure.}},
 FJournal = {{Inventiones Mathematicae}},
 Journal = {{Invent. Math.}},
 ISSN = {0020-9910; 1432-1297/e},
 Volume = {217},
 Number = {3},
 Pages = {749--797},
 Year = {2019},
 Publisher = {Springer, Berlin/Heidelberg},
 Language = {English},
 MSC2010 = {37F45 37F10 32G15 37P45}
}


@Article{vS00,
 Author = {Sebastian {van Strien}},
 Title = {{Misiurewicz maps unfold generically (even if they are critically non-finite).}},
 FJournal = {{Fundamenta Mathematicae}},
 Journal = {{Fundam. Math.}},
 ISSN = {0016-2736; 1730-6329/e},
 Volume = {163},
 Number = {1},
 Pages = {39--54},
 Year = {2000},
 Publisher = {Polish Academy of Sciences (Polska Akademia Nauk - PAN), Institute of Mathematics (Instytut Matematyczny), Warsaw},
 Language = {English},
 MSC2010 = {37F45 37E05 37G99 37C15},
 Zbl = {0965.37038}
}

@article{Ru01,
author = {Ruelle, David},
year = {2001},
month = {06},
pages = {},
title = {Historical behaviour in smooth dynamical systems},
doi = {10.1201/9781420034288.ch2}
}

@article{KYT19,
author = {Kiriki, Shin and Nakano, Yushi and Soma, Teruhiko},
year = {2019},
pages = {1111-1124},
title = {Historic behaviour for nonautonomous contraction mappings},
volume = {32},
journal = {Nonlinearity},
doi = {10.1088/1361-6544/aaf253}
}
@article{KLS16,
author = {Kiriki, Shin and Li, Ming-Chia and Soma, Teruhiko},
year = {2016},
month = {12},
pages = {},
title = {Geometric Lorenz flows with historic behavior},
volume = {36},
journal = {Discrete and Continuous Dynamical Systems -A},
doi = {10.3934/dcds.2016105}
}

@unknown{CYZ18,
author = {Crovisier, Sylvain and Yang, Dawei and Zhang, Jinhua},
year = {2018},
month = {11},
pages = {},
title = {Empirical measures of partially hyperbolic attractors}
}

@incollection{FH77,
     author = {Fathi, Albert and Herman, Michael R.},
     title = {Existence de diff\'eomorphismes minimaux},
     booktitle = {Syst\`eme dynamique I - Varsovie},
     author = {Collectif},
     series = {Ast\'erisque},
     publisher = {Soci\'et\'e math\'ematique de France},
     number = {49},
     year = {1977},
     pages = {37-59},
     zbl = {0374.58010},
     mrnumber = {482843},
     language = {fr},
     url = {http://www.numdam.org/item/AST_1977__49__37_0}
}


@article{AK70,
author = {Anosov, D.V. and Katok, A.B.},
year = {1970},
month = {01},
pages = {},
title = {New examples in smooth ergodic theory. Ergodic diffeomorphisms},
volume = {23},
journal = {Transactions of the Moscow Mathematical Society}
}

@InCollection{McMullen,
 Author = {Curtis T. {McMullen}},
 Title = {{The Mandelbrot set is universal.}},
 BookTitle = {{The Mandelbrot set, theme and variations}},
 ISBN = {0-521-77476-4/pbk},
 Pages = {1--17},
 Year = {2000},
 Publisher = {Cambridge: Cambridge University Press},
 Language = {English},
 MSC2010 = {37F45 37F10 30D05},
 Zbl = {1062.37042}
}
